Crop identification using deep learning on LUCAS crop cover photos

Crop classification via deep learning on ground imagery can deliver timely and accurate crop-specific information to various stakeholders. Dedicated ground-based image acquisition exercises can help to collect data in data scarce regions, improve control on timing of collection, or when study areas are to small to monitor via satellite. Automatic labelling is essential when collecting large volumes of data. One such data collection is the EU's Land Use Cover Area frame Survey (LUCAS), and in particular, the recently published LUCAS Cover photos database. The aim of this paper is to select and publish a subset of LUCAS Cover photos for 12 mature major crops across the EU, to deploy, benchmark, and identify the best configuration of Mobile-net for the classification task, to showcase the possibility of using entropy-based metrics for post-processing of results, and finally to show the applications and limitations of the model in a practical and policy relevant context. In particular, the usefulness of automatically identifying crops on geo-tagged photos is illustrated in the context of the EU's Common Agricultural Policy. The work has produced a dataset of 169,460 images of mature crops for the 12 classes, out of which 15,876 were manually selected as representing a clean sample without any foreign objects or unfavorable conditions. The best performing model achieved a Macro F1 (M-F1) of 0.75 on an imbalanced test dataset of 8,642 photos. Using metrics from information theory, namely - the Equivalence Reference Probability, resulted in achieving an increase of 6%. The most unfavorable conditions for taking such images, across all crop classes, were found to be too early or late in the season. The proposed methodology shows the possibility for using minimal auxiliary data, outside the images themselves, in order to achieve a M-F1 of 0.817 for labelling between 12 major European crops.

==> tables/Results__crop_photos_june_6class_n100_mobilenet_05_224_assesment_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 18:49:35 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA & 484 &  25 &  71 &  22 &  54 &  55 & 711 \\ 
  MAI &  27 & 296 &  26 &  89 &  83 &  23 & 544 \\ 
  ONI &  60 &  31 & 423 &  80 &  70 &  40 & 704 \\ 
  POT &  30 &  79 &  40 & 480 & 126 &  58 & 813 \\ 
  SBT &  38 &  66 &  26 & 116 & 433 &  54 & 733 \\ 
  WWH &  50 &  23 &  28 &  37 &  59 & 305 & 502 \\ 
  TOTAL & 689 & 520 & 614 & 824 & 825 & 535 & 4007 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n100_mobilenet_05_224_assesment_FIELD_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 18:49:37 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA &  24 &   0 &   2 &   0 &   1 &   0 &  27 \\ 
  MAI &   0 &  19 &   1 &   2 &   3 &   0 &  25 \\ 
  ONI &   1 &   0 &  18 &   3 &   2 &   0 &  24 \\ 
  POT &   0 &   1 &   0 &  21 &   3 &   2 &  27 \\ 
  SBT &   1 &   1 &   0 &   3 &  23 &   0 &  28 \\ 
  WWH &   1 &   1 &   0 &   0 &   2 &  15 &  19 \\ 
  TOTAL &  27 &  22 &  21 &  29 &  34 &  17 & 150 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n100_mobilenet_05_224_assesment_FIELD_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 18:49:37 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.89 & 0.89 & 0.89 \\ 
  MAI & 0.86 & 0.76 & 0.81 \\ 
  ONI & 0.86 & 0.75 & 0.80 \\ 
  POT & 0.72 & 0.78 & 0.75 \\ 
  SBT & 0.68 & 0.82 & 0.74 \\ 
  WWH & 0.88 & 0.79 & 0.83 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n100_mobilenet_05_224_assesment_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 18:49:35 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.70 & 0.68 & 0.69 \\ 
  MAI & 0.57 & 0.54 & 0.56 \\ 
  ONI & 0.69 & 0.60 & 0.64 \\ 
  POT & 0.58 & 0.59 & 0.59 \\ 
  SBT & 0.52 & 0.59 & 0.56 \\ 
  WWH & 0.57 & 0.61 & 0.59 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n100_mobilenet_1_224_assesment_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 19:00:25 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA & 558 &  24 &  58 &  16 &  18 &  37 & 711 \\ 
  MAI &  12 & 394 &  17 &  59 &  48 &  14 & 544 \\ 
  ONI &  41 &  25 & 548 &  36 &  31 &  23 & 704 \\ 
  POT &  14 &  87 &  45 & 534 &  78 &  55 & 813 \\ 
  SBT &  24 &  70 &  12 &  93 & 479 &  55 & 733 \\ 
  WWH &  29 &  10 &  14 &  23 &  32 & 394 & 502 \\ 
  TOTAL & 678 & 610 & 694 & 761 & 686 & 578 & 4007 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n100_mobilenet_1_224_assesment_FIELD_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 19:00:26 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA &  26 &   0 &   1 &   0 &   0 &   0 &  27 \\ 
  MAI &   0 &  23 &   0 &   1 &   1 &   0 &  25 \\ 
  ONI &   0 &   0 &  22 &   1 &   1 &   0 &  24 \\ 
  POT &   0 &   2 &   0 &  23 &   1 &   1 &  27 \\ 
  SBT &   1 &   1 &   0 &   2 &  24 &   0 &  28 \\ 
  WWH &   0 &   0 &   0 &   0 &   2 &  17 &  19 \\ 
  TOTAL &  27 &  26 &  23 &  27 &  29 &  18 & 150 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n100_mobilenet_1_224_assesment_FIELD_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 19:00:26 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.96 & 0.96 & 0.96 \\ 
  MAI & 0.88 & 0.92 & 0.90 \\ 
  ONI & 0.96 & 0.92 & 0.94 \\ 
  POT & 0.85 & 0.85 & 0.85 \\ 
  SBT & 0.83 & 0.86 & 0.84 \\ 
  WWH & 0.94 & 0.89 & 0.92 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n100_mobilenet_1_224_assesment_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 19:00:25 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.82 & 0.78 & 0.80 \\ 
  MAI & 0.65 & 0.72 & 0.68 \\ 
  ONI & 0.79 & 0.78 & 0.78 \\ 
  POT & 0.70 & 0.66 & 0.68 \\ 
  SBT & 0.70 & 0.65 & 0.68 \\ 
  WWH & 0.68 & 0.78 & 0.73 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n200_mobilenet_05_224_assesment_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 19:05:16 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA & 484 &  25 &  71 &  22 &  54 &  55 & 711 \\ 
  MAI &  27 & 296 &  26 &  89 &  83 &  23 & 544 \\ 
  ONI &  60 &  31 & 423 &  80 &  70 &  40 & 704 \\ 
  POT &  30 &  79 &  40 & 480 & 126 &  58 & 813 \\ 
  SBT &  38 &  66 &  26 & 116 & 433 &  54 & 733 \\ 
  WWH &  50 &  23 &  28 &  37 &  59 & 305 & 502 \\ 
  TOTAL & 689 & 520 & 614 & 824 & 825 & 535 & 4007 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n200_mobilenet_05_224_assesment_FIELD_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 19:05:18 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA &  24 &   0 &   2 &   0 &   1 &   0 &  27 \\ 
  MAI &   0 &  19 &   1 &   2 &   3 &   0 &  25 \\ 
  ONI &   1 &   0 &  18 &   3 &   2 &   0 &  24 \\ 
  POT &   0 &   1 &   0 &  21 &   3 &   2 &  27 \\ 
  SBT &   1 &   1 &   0 &   3 &  23 &   0 &  28 \\ 
  WWH &   1 &   1 &   0 &   0 &   2 &  15 &  19 \\ 
  TOTAL &  27 &  22 &  21 &  29 &  34 &  17 & 150 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n200_mobilenet_05_224_assesment_FIELD_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 19:05:18 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.89 & 0.89 & 0.89 \\ 
  MAI & 0.86 & 0.76 & 0.81 \\ 
  ONI & 0.86 & 0.75 & 0.80 \\ 
  POT & 0.72 & 0.78 & 0.75 \\ 
  SBT & 0.68 & 0.82 & 0.74 \\ 
  WWH & 0.88 & 0.79 & 0.83 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n200_mobilenet_05_224_assesment_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 19:05:16 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.70 & 0.68 & 0.69 \\ 
  MAI & 0.57 & 0.54 & 0.56 \\ 
  ONI & 0.69 & 0.60 & 0.64 \\ 
  POT & 0.58 & 0.59 & 0.59 \\ 
  SBT & 0.52 & 0.59 & 0.56 \\ 
  WWH & 0.57 & 0.61 & 0.59 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n200_mobilenet_1_224_assesment_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 20:02:56 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA & 493 &   6 &  45 &  15 &  18 &  34 & 611 \\ 
  MAI &  11 & 358 &  17 &  34 &  14 &  10 & 444 \\ 
  ONI &  57 &  16 & 483 &  19 &   9 &  20 & 604 \\ 
  POT &   4 &  80 &  51 & 507 &  46 &  25 & 713 \\ 
  SBT &  25 &  64 &  15 &  71 & 433 &  25 & 633 \\ 
  WWH &  13 &   5 &   9 &  14 &  15 & 346 & 402 \\ 
  TOTAL & 603 & 529 & 620 & 660 & 535 & 460 & 3407 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n200_mobilenet_1_224_assesment_FIELD_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 20:02:58 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA &  26 &   0 &   1 &   0 &   0 &   0 &  27 \\ 
  MAI &   0 &  25 &   0 &   0 &   0 &   0 &  25 \\ 
  ONI &   2 &   0 &  21 &   0 &   0 &   1 &  24 \\ 
  POT &   0 &   0 &   1 &  26 &   0 &   0 &  27 \\ 
  SBT &   1 &   1 &   0 &   1 &  25 &   0 &  28 \\ 
  WWH &   0 &   0 &   0 &   0 &   1 &  18 &  19 \\ 
  TOTAL &  29 &  26 &  23 &  27 &  26 &  19 & 150 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n200_mobilenet_1_224_assesment_FIELD_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 20:02:58 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.90 & 0.96 & 0.93 \\ 
  MAI & 0.96 & 1.00 & 0.98 \\ 
  ONI & 0.91 & 0.88 & 0.89 \\ 
  POT & 0.96 & 0.96 & 0.96 \\ 
  SBT & 0.96 & 0.89 & 0.93 \\ 
  WWH & 0.95 & 0.95 & 0.95 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n200_mobilenet_1_224_assesment_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 20:02:56 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.82 & 0.81 & 0.81 \\ 
  MAI & 0.68 & 0.81 & 0.74 \\ 
  ONI & 0.78 & 0.80 & 0.79 \\ 
  POT & 0.77 & 0.71 & 0.74 \\ 
  SBT & 0.81 & 0.68 & 0.74 \\ 
  WWH & 0.75 & 0.86 & 0.80 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n300_mobilenet_05_224_assesment_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 19:47:13 2018
\begin{table}[ht]
\centering
\begin{tabular}{rr}
  \hline
 & TOTAL \\ 
  \hline
TOTAL &   0 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n300_mobilenet_05_224_assesment_FIELD_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 17:33:18 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA &  23 &   0 &   1 &   0 &   1 &   2 &  27 \\ 
  MAI &   0 &  24 &   0 &   0 &   1 &   0 &  25 \\ 
  ONI &   1 &   1 &  21 &   0 &   0 &   1 &  24 \\ 
  POT &   1 &  13 &   1 &   5 &   4 &   3 &  27 \\ 
  SBT &   1 &   3 &   0 &   0 &  23 &   1 &  28 \\ 
  WWH &   0 &   1 &   0 &   0 &   0 &  18 &  19 \\ 
  TOTAL &  26 &  42 &  23 &   5 &  29 &  25 & 150 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n300_mobilenet_05_224_assesment_FIELD_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 17:33:18 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.88 & 0.85 & 0.87 \\ 
  MAI & 0.57 & 0.96 & 0.72 \\ 
  ONI & 0.91 & 0.88 & 0.89 \\ 
  POT & 1.00 & 0.19 & 0.31 \\ 
  SBT & 0.79 & 0.82 & 0.81 \\ 
  WWH & 0.72 & 0.95 & 0.82 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n300_mobilenet_05_224_assesment_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Fri Nov 16 17:33:17 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.82 & 0.64 & 0.72 \\ 
  MAI & 0.41 & 0.85 & 0.55 \\ 
  ONI & 0.76 & 0.72 & 0.74 \\ 
  POT & 0.85 & 0.19 & 0.31 \\ 
  SBT & 0.67 & 0.71 & 0.69 \\ 
  WWH & 0.49 & 0.81 & 0.61 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n300_mobilenet_1_224_assesment_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 09:53:46 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA & 473 &   3 &  12 &   0 &   7 &  16 & 511 \\ 
  MAI &   0 & 317 &   6 &  12 &   8 &   1 & 344 \\ 
  ONI &  10 &   3 & 481 &   5 &   3 &   2 & 504 \\ 
  POT &   0 &  16 &  13 & 550 &  22 &  12 & 613 \\ 
  SBT &   8 &  13 &   5 &  24 & 475 &   8 & 533 \\ 
  WWH &   1 &   0 &   2 &   8 &   3 & 288 & 302 \\ 
  TOTAL & 492 & 352 & 519 & 599 & 518 & 327 & 2807 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n300_mobilenet_1_224_assesment_FIELD_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 09:53:49 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA &  27 &   0 &   0 &   0 &   0 &   0 &  27 \\ 
  MAI &   0 &  25 &   0 &   0 &   0 &   0 &  25 \\ 
  ONI &   0 &   0 &  24 &   0 &   0 &   0 &  24 \\ 
  POT &   0 &   0 &   0 &  26 &   1 &   0 &  27 \\ 
  SBT &   0 &   0 &   0 &   0 &  28 &   0 &  28 \\ 
  WWH &   0 &   0 &   0 &   0 &   0 &  19 &  19 \\ 
  TOTAL &  27 &  25 &  24 &  26 &  29 &  19 & 150 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n300_mobilenet_1_224_assesment_FIELD_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 09:53:49 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 1.00 & 1.00 & 1.00 \\ 
  MAI & 1.00 & 1.00 & 1.00 \\ 
  ONI & 1.00 & 1.00 & 1.00 \\ 
  POT & 1.00 & 0.96 & 0.98 \\ 
  SBT & 0.97 & 1.00 & 0.98 \\ 
  WWH & 1.00 & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n300_mobilenet_1_224_assesment_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 09:53:46 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.96 & 0.93 & 0.94 \\ 
  MAI & 0.90 & 0.92 & 0.91 \\ 
  ONI & 0.93 & 0.95 & 0.94 \\ 
  POT & 0.92 & 0.90 & 0.91 \\ 
  SBT & 0.92 & 0.89 & 0.90 \\ 
  WWH & 0.88 & 0.95 & 0.92 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n400_mobilenet_05_224_assesment_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 10:20:31 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA & 353 &  10 &   9 &  21 &   3 &  15 & 411 \\ 
  MAI &  13 & 167 &   3 &  48 &   5 &   8 & 244 \\ 
  ONI &  75 &  19 & 225 &  47 &   3 &  35 & 404 \\ 
  POT &  29 &  41 &  13 & 403 &   9 &  18 & 513 \\ 
  SBT &  53 &  57 &   8 & 172 & 119 &  24 & 433 \\ 
  WWH &  21 &   7 &   3 &  16 &   0 & 155 & 202 \\ 
  TOTAL & 544 & 301 & 261 & 707 & 139 & 255 & 2207 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n400_mobilenet_05_224_assesment_FIELD_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 10:20:33 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA &  27 &   0 &   0 &   0 &   0 &   0 &  27 \\ 
  MAI &   0 &  19 &   0 &   6 &   0 &   0 &  25 \\ 
  ONI &   5 &   0 &  17 &   1 &   0 &   1 &  24 \\ 
  POT &   0 &   1 &   0 &  26 &   0 &   0 &  27 \\ 
  SBT &   3 &   2 &   0 &  15 &   7 &   1 &  28 \\ 
  WWH &   0 &   0 &   0 &   1 &   0 &  18 &  19 \\ 
  TOTAL &  35 &  22 &  17 &  49 &   7 &  20 & 150 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n400_mobilenet_05_224_assesment_FIELD_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 10:20:33 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.77 & 1.00 & 0.87 \\ 
  MAI & 0.86 & 0.76 & 0.81 \\ 
  ONI & 1.00 & 0.71 & 0.83 \\ 
  POT & 0.53 & 0.96 & 0.68 \\ 
  SBT & 1.00 & 0.25 & 0.40 \\ 
  WWH & 0.90 & 0.95 & 0.92 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n400_mobilenet_05_224_assesment_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 10:20:31 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.65 & 0.86 & 0.74 \\ 
  MAI & 0.55 & 0.68 & 0.61 \\ 
  ONI & 0.86 & 0.56 & 0.68 \\ 
  POT & 0.57 & 0.79 & 0.66 \\ 
  SBT & 0.86 & 0.27 & 0.42 \\ 
  WWH & 0.61 & 0.77 & 0.68 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n400_mobilenet_1_224_assesment_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 10:35:07 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA & 364 &   4 &  13 &   8 &   8 &  14 & 411 \\ 
  MAI &   5 & 201 &   4 &  15 &  13 &   6 & 244 \\ 
  ONI &  33 &   8 & 337 &  15 &   3 &   8 & 404 \\ 
  POT &   4 &  24 &  12 & 428 &  34 &  11 & 513 \\ 
  SBT &   9 &  29 &   6 &  49 & 321 &  19 & 433 \\ 
  WWH &   4 &   4 &   4 &   8 &  13 & 169 & 202 \\ 
  TOTAL & 419 & 270 & 376 & 523 & 392 & 227 & 2207 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n400_mobilenet_1_224_assesment_FIELD_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 10:35:08 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA &  27 &   0 &   0 &   0 &   0 &   0 &  27 \\ 
  MAI &   0 &  24 &   0 &   1 &   0 &   0 &  25 \\ 
  ONI &   0 &   0 &  24 &   0 &   0 &   0 &  24 \\ 
  POT &   0 &   0 &   0 &  27 &   0 &   0 &  27 \\ 
  SBT &   0 &   0 &   0 &   1 &  27 &   0 &  28 \\ 
  WWH &   0 &   0 &   0 &   0 &   0 &  19 &  19 \\ 
  TOTAL &  27 &  24 &  24 &  29 &  27 &  19 & 150 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n400_mobilenet_1_224_assesment_FIELD_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 10:35:08 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 1.00 & 1.00 & 1.00 \\ 
  MAI & 1.00 & 0.96 & 0.98 \\ 
  ONI & 1.00 & 1.00 & 1.00 \\ 
  POT & 0.93 & 1.00 & 0.96 \\ 
  SBT & 1.00 & 0.96 & 0.98 \\ 
  WWH & 1.00 & 1.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n400_mobilenet_1_224_assesment_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 10:35:07 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.87 & 0.89 & 0.88 \\ 
  MAI & 0.74 & 0.82 & 0.78 \\ 
  ONI & 0.90 & 0.83 & 0.86 \\ 
  POT & 0.82 & 0.83 & 0.83 \\ 
  SBT & 0.82 & 0.74 & 0.78 \\ 
  WWH & 0.74 & 0.84 & 0.79 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n500_mobilenet_05_224_assesment_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 10:51:41 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA & 252 &   1 &  20 &  14 &  24 &   0 & 311 \\ 
  MAI &   9 &  46 &   8 &  55 &  26 &   0 & 144 \\ 
  ONI &  26 &   0 & 221 &  33 &  24 &   0 & 304 \\ 
  POT &  11 &   6 &  18 & 325 &  53 &   0 & 413 \\ 
  SBT &  16 &   2 &   7 &  64 & 244 &   0 & 333 \\ 
  WWH &  25 &   1 &  13 &  29 &  15 &  19 & 102 \\ 
  TOTAL & 339 &  56 & 287 & 520 & 386 &  19 & 1607 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n500_mobilenet_05_224_assesment_FIELD_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 10:51:43 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA &  27 &   0 &   0 &   0 &   0 &   0 &  27 \\ 
  MAI &   1 &   8 &   1 &   9 &   6 &   0 &  25 \\ 
  ONI &   2 &   0 &  19 &   3 &   0 &   0 &  24 \\ 
  POT &   0 &   0 &   0 &  27 &   0 &   0 &  27 \\ 
  SBT &   1 &   0 &   0 &   5 &  22 &   0 &  28 \\ 
  WWH &   2 &   0 &   2 &   7 &   3 &   5 &  19 \\ 
  TOTAL &  33 &   8 &  22 &  51 &  31 &   5 & 150 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n500_mobilenet_05_224_assesment_FIELD_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 10:51:43 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.82 & 1.00 & 0.90 \\ 
  MAI & 1.00 & 0.32 & 0.48 \\ 
  ONI & 0.86 & 0.79 & 0.83 \\ 
  POT & 0.53 & 1.00 & 0.69 \\ 
  SBT & 0.71 & 0.79 & 0.75 \\ 
  WWH & 1.00 & 0.26 & 0.42 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n500_mobilenet_05_224_assesment_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Mon Nov 19 10:51:41 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.74 & 0.81 & 0.78 \\ 
  MAI & 0.82 & 0.32 & 0.46 \\ 
  ONI & 0.77 & 0.73 & 0.75 \\ 
  POT & 0.62 & 0.79 & 0.70 \\ 
  SBT & 0.63 & 0.73 & 0.68 \\ 
  WWH & 1.00 & 0.19 & 0.31 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n500_mobilenet_1_224_assesment_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 11:06:21 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA & 276 &   6 &  18 &   2 &   5 &   4 & 311 \\ 
  MAI &   3 & 123 &   4 &   8 &   3 &   3 & 144 \\ 
  ONI &  13 &   6 & 267 &   5 &   9 &   4 & 304 \\ 
  POT &   4 &  32 &  11 & 337 &  20 &   9 & 413 \\ 
  SBT &   7 &  20 &   9 &  26 & 264 &   7 & 333 \\ 
  WWH &   5 &   4 &   3 &   6 &   5 &  79 & 102 \\ 
  TOTAL & 308 & 191 & 312 & 384 & 306 & 106 & 1607 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n500_mobilenet_1_224_assesment_FIELD_CM.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 11:06:23 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrr}
  \hline
 & GRA & MAI & ONI & POT & SBT & WWH & TOTAL \\ 
  \hline
GRA &  27 &   0 &   0 &   0 &   0 &   0 &  27 \\ 
  MAI &   1 &  23 &   0 &   0 &   0 &   0 &  24 \\ 
  ONI &   0 &   0 &  24 &   0 &   0 &   0 &  24 \\ 
  POT &   0 &   0 &   0 &  27 &   0 &   0 &  27 \\ 
  SBT &   1 &   1 &   0 &   0 &  26 &   0 &  28 \\ 
  WWH &   0 &   1 &   0 &   0 &   0 &  18 &  19 \\ 
  TOTAL &  29 &  25 &  24 &  27 &  26 &  18 & 149 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n500_mobilenet_1_224_assesment_FIELD_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 11:06:23 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.93 & 1.00 & 0.96 \\ 
  MAI & 0.92 & 0.96 & 0.94 \\ 
  ONI & 1.00 & 1.00 & 1.00 \\ 
  POT & 1.00 & 1.00 & 1.00 \\ 
  SBT & 1.00 & 0.93 & 0.96 \\ 
  WWH & 1.00 & 0.95 & 0.97 \\ 
   \hline
\end{tabular}
\end{table}


==> tables/Results__crop_photos_june_6class_n500_mobilenet_1_224_assesment_perClass.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-2 package
% Tue Nov 20 11:06:21 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & UA & PA & F\_score \\ 
  \hline
GRA & 0.90 & 0.89 & 0.89 \\ 
  MAI & 0.64 & 0.85 & 0.73 \\ 
  ONI & 0.86 & 0.88 & 0.87 \\ 
  POT & 0.88 & 0.82 & 0.85 \\ 
  SBT & 0.86 & 0.79 & 0.83 \\ 
  WWH & 0.75 & 0.77 & 0.76 \\ 
   \hline
\end{tabular}
\end{table}

